End-To-End Real-Time Visual Perception Framework for Construction Automation

In this work, we present a robotic solution to automate the task of wall construction. To that end, we present an end-to-end visual perception framework that can quickly detect and localize bricks in a clutter. Further, we present a light computational method of brick pose estimation that incorporates the above information. The proposed detection network predicts a rotated box compared to YOLO and SSD, thereby maximizing the object's region in the predicted box regions. In addition, precision P, recall R, and mean-average-precision (mAP) scores are reported to evaluate the proposed framework. We observed that for our task, the proposed scheme outperforms the upright bounding box detectors. Further, we deploy the proposed visual perception framework on a robotic system endowed with a UR5 robot manipulator and demonstrate that the system can successfully replicate a simplified version of the wall-building task in an autonomous mode.

==> poseEstimation.tex <==
\section{Pose Estimation}

\label{sec_pose}
In this section we will estimate the 6D pose of the brick. We observed that for a cubical shape object at least four corner points are sufficient to estimate the 6D pose of the object \textit{i.e.} if we know 3D coordinates of four corner points of the brick, then we can estimate the 6-\textit{DOF} pose of the brick. To estimate the corners of the brick, first we feed the current image (Fig. \ref{fig:pose1}) to the rotating box network. Region corresponding to the rotating box (Fig. \ref{fig:brick_seg}) is called brick region and point cloud corresponding to the the brick region is called brick cloud. In brick cloud, we estimate the edge points (\ref{fig:edges}), then using RANSAC method we fit the line on the edges (\ref{fig:lines}) and intersection of lines will give the corner points. From the corner points we estimate the pose of the brick as shown in Fig. \ref{fig:pose}.



\begin{figure}[t]
    \centering
\begin{subfigure}{0.125\textwidth}
  \includegraphics[width=1.18\linewidth]{images/pose_estimation/sample.jpg}
  \caption{Image}
  \label{fig:pose1}
\end{subfigure}\hfil
\begin{subfigure}{0.125\textwidth}
  \includegraphics[width=1.18\linewidth]{images/pose_estimation/bb_box_pose.jpg}
  \caption{Rotating box}
  \label{fig:brick_seg}
\end{subfigure}\hfil
\begin{subfigure}{0.125\textwidth}
  \includegraphics[height=0.89\linewidth, width=1.15\linewidth]{images/pose_estimation/real_cloud.jpg}
  \caption{Point Cloud}
\end{subfigure}

\medskip
\begin{subfigure}{0.125\textwidth}
  \includegraphics[height=0.89\linewidth, width=1.16\linewidth]{images/pose_estimation/edges.jpg}
  \caption{Edges}
  \label{fig:edges}
\end{subfigure}\hfil
\begin{subfigure}{0.125\textwidth}
  \includegraphics[height=0.89\linewidth, width=1.16\linewidth]{images/pose_estimation/lines.jpg}
  \caption{Lines}
  \label{fig:lines}
\end{subfigure}\hfil
\begin{subfigure}{0.125\textwidth}
  \includegraphics[height=0.89\linewidth, width=1.15\linewidth]{images/pose_estimation/pose.jpg}
  \caption{6D Pose}
  \label{fig:pose}
\end{subfigure}
\caption{Pose estimation pipeline}
  \label{fig:complete_pose}
    \vspace{-4mm}
\end{figure}
